Eluder-based Regret for Stochastic Contextual MDPs

We present the E-UC$^3$RL algorithm for regret minimization in Stochastic Contextual Markov Decision Processes (CMDPs). The algorithm operates under the minimal assumptions of realizable function class and access to \emph{offline} least squares and log loss regression oracles. Our algorithm is efficient (assuming efficient offline regression oracles) and enjoys a regret guarantee of $ \widetilde{O}(H^3 \sqrt{T |S| |A|d_{\mathrm{E}}(\mathcal{P}) \log (|\mathcal{F}| |\mathcal{P}|/ \delta) )}) , $ with $T$ being the number of episodes, $S$ the state space, $A$ the action space, $H$ the horizon, $\mathcal{P}$ and $\mathcal{F}$ are finite function classes used to approximate the context-dependent dynamics and rewards, respectively, and $d_{\mathrm{E}}(\mathcal{P})$ is the Eluder dimension of $\mathcal{P}$ w.r.t the Hellinger distance. To the best of our knowledge, our algorithm is the first efficient and rate-optimal regret minimization algorithm for CMDPs that operates under the general offline function approximation setting. In addition, we extend the Eluder dimension to general bounded metrics which may be of separate interest.

==> mathdefs.tex <==
%%Requeiried packages and preliminary definitions, needed by the options
\RequirePackage{mathtools}
% \RequirePackage{thmtools}
% \RequirePackage{amsfonts}
\RequirePackage{dsfont}
\RequirePackage{delimset}

%%Body of the package, most of the declarations appear here.

\newcommand{\R}{\mathbb{R}} %reals
\newcommand{\N}{\mathbb{N}} % naturals
%\newcommand{\Reg}{\text{E.Regret}}
\newcommand{\Regrv}{\mathcal{R}}

\newcommand{\Reals}{\mathbb{R}} %reals
\newcommand{\Naturals}{\mathbb{N}} % naturals
\newcommand{\Var}{\mathbb{V}}%Variance
\newcommand{\E}{\mathbb{E}} % expectation
\newcommand{\Prob}{\mathbb{P}} % probability

\newcommand{\I}{\mathbb{I}} %indicator
\newcommand{\B}{\mathcal{B}} %Bernoulli rv
\newcommand{\V}{\mathbb{V}} % variance






\newcommand{\innProd}[2][*]{\brk[a]#1{#2}}
\newcommand{\ceil}[2][*]{\delim\lceil\rceil#1{#2}}
\newcommand{\floor}[2][*]{\delim\lfloor\rfloor#1{#2}}
\newcommand{\indEvent}[2][*]{\I_{\brk[c]#1{#2}}}
% \newcommand{\indEvent}[2][*]{\mathbb{1}{\brk[c]#1{#2}}}
\newcommand{\indFunc}[2][\infty]{\I_{\brk[s]{#2,#1}}}
\newcommand{\indFuncAt}[3][\infty]{\indFunc[#1]{#2}\brk*{#3}}
\newcommand{\tr}[2][*]{\mathrm{Tr}\brk*{#2}}
\newcommand{\overbar}[1]{\mkern 2mu\overline{\mkern-2mu#1\mkern-2mu}\mkern 2mu}
\newcommand{\tran}{^{\mkern-1.5mu\mathsf{T}}}


% Standard Math Notations
\newcommand{\Oof}[2][*]{O\brk#1{#2}}
\newcommand{\OtildeOf}[2][*]{\smash{\widetilde{O}}\brk#1{#2}}

\newcommand{\poly}{\mathrm{poly}}



% Probability
\newcommand{\gaussDist}[2]{\mathcal{N}\brk0{#1, #2}}

% Math operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}



% General
\def\noi{\noindent}

\newcommand{\ifrac}[2]{#1/#2}

\newcommand{\rootT}{\ensuremath{\smash{\sqrt{T}}}\xspace}

==> thmdefs.tex <==
%%Requeiried packages and preliminary definitions, needed by the options
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{thmtools}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREM STYLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%% standard

% \declaretheoremstyle[
% 	    spaceabove=\topsep, 
% 	    spacebelow=\topsep, 
% 	    bodyfont=\normalfont\itshape,
%     ]{theorem}

% \declaretheorem[style=theorem,name=Theorem]{theorem}

% \declaretheoremstyle[
% 	    spaceabove=\topsep, 
% 	    spacebelow=\topsep, 
% 	    bodyfont=\normalfont,
%     ]{definition}
    
%%%%%% JMLR-style

\setlength{\topsep}{\medskipamount}

\declaretheoremstyle[
	    spaceabove=\topsep, 
	    spacebelow=\topsep, 
	    headfont=\normalfont\bfseries,
	    bodyfont=\normalfont\itshape,
	    notefont=\normalfont\bfseries,
	    notebraces={(}{)},
	    postheadspace=0.33em, 
	    headpunct={.},
	   % postfoothook=\noindent\ignorespaces
    ]{theorem}
% \declaretheorem[style=theorem,numberwithin=section]{theorem}
\declaretheorem[style=theorem]{theorem}

\declaretheoremstyle[
	    spaceabove=\topsep, 
	    spacebelow=\topsep, 
	    headfont=\normalfont\bfseries,
	    bodyfont=\normalfont,
	    notefont=\normalfont\bfseries,
	    notebraces={(}{)},
	    postheadspace=0.33em, 
	    headpunct={.},
	   % postfoothook=\noindent\ignorespaces
    ]{definition}

\let\proof\undefined
\declaretheoremstyle[
        spaceabove=\topsep, 
        spacebelow=\topsep, 
        headfont=\normalfont\bfseries,
        bodyfont=\normalfont,
        notefont=\normalfont\bfseries,
        % notebraces={(}{)},
        notebraces={}{},
        postheadspace=0.33em, 
        qed=$\blacksquare$, 
        headpunct={.},
        % postfoothook=\noindent\ignorespaces
    ]{proofstyle}
\declaretheorem[style=proofstyle,numbered=no,name=Proof]{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		
% \declaretheorem[style=theorem,sibling=theorem,name=Lemma]{lemma}
% \declaretheorem[style=theorem,sibling=theorem,name=Corollary]{corollary}
% \declaretheorem[style=theorem,sibling=theorem,name=Claim]{claim}
% \declaretheorem[style=theorem,sibling=theorem,name=Proposition]{proposition}
% \declaretheorem[style=theorem,sibling=theorem,name=Fact]{fact}
% \declaretheorem[style=theorem,sibling=theorem,name=Observation]{observation}
% \declaretheorem[style=theorem,sibling=theorem,name=Conjecture]{conjecture}

\declaretheorem[style=theorem,numbered=no,name=Theorem]{theorem*}
\declaretheorem[style=theorem,numbered=no,name=Lemma]{lemma*}
\declaretheorem[style=theorem,numbered=no,name=Corollary]{corollary*}
\declaretheorem[style=theorem,numbered=no,name=Proposition]{proposition*}
\declaretheorem[style=theorem,numbered=no,name=Claim]{claim*}
\declaretheorem[style=theorem,numbered=no,name=Fact]{fact*}
\declaretheorem[style=theorem,numbered=no,name=Observation]{observation*}
\declaretheorem[style=theorem,numbered=no,name=Conjecture]{conjecture*}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,sibling=theorem,name=Remark]{remark}
\declaretheorem[style=definition,sibling=theorem,name=Example]{example}
\declaretheorem[style=definition,sibling=theorem,name=Question]{question}

\declaretheorem[style=definition,numbered=no,name=Definition]{definition*}
\declaretheorem[style=definition,numbered=no,name=Remark]{remark*}
\declaretheorem[style=definition,numbered=no,name=Example]{example*}
\declaretheorem[style=definition,numbered=no,name=Question]{question*}

\declaretheorem[style=theorem,sibling=theorem,name=Assumption]{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
